Setting the cornerstone for the IMRPhenomX family of models for gravitational waves from compact binaries: The dominant harmonic for non-precessing quasi-circular black holes

In this paper we present IMRPhenomXAS, a thorough overhaul of the IMRPhenomD [1,2] waveform model, which describes the dominant $l=2, \:| m | = 2$ spherical harmonic mode of non-precessing coalescing black holes in terms of piecewise closed form expressions in the frequency domain. Improvements include in particular the accurate treatment of unequal spin effects, and the inclusion of extreme mass ratio waveforms. IMRPhenomD has previously been extended to approximately include spin precession [3] and subdominant spherical harmonics [4], and with its extensions it has become a standard tool in gravitational wave parameter estimation. Improved extensions of IMRPhenomXAS are discussed in companion papers [5,6].

==> Preamble.tex <==
%auto-ignore

\makeatletter

%% Smaller space between section number and name
\def\@seccntformat#1{\csname the#1\endcsname.~}%

%% Smaller space between preceding text and new section headings
\def\section{%
  \@startsection {section}
  {1} {\z@} {0.55cm \@plus1ex \@minus .02ex}%
    {0.225cm} { \normalfont\bfseries \centering}%
}%
\def\subsection{%
  \@startsection {subsection}
  {2} {\z@ } {0.45cm \@plus 0.8ex \@minus 0.2ex}%
  {0.1125cm}{\normalfont \bfseries \centering }}
\def\subsubsection{%
  \@startsection {subsubsection}
  {3} {\z@ } {0.4cm \@plus 0.6ex \@minus 0.1ex}%
  {0.075cm}{\normalfont \it \centering }}

%% Headers and footers
\newcommand{\surnames}[1]{\def\@surnamelist{#1}\relax}
\surnames{\ }
\ifx \@shorttitle \@empty
  % \def\@oddhead{\small \MakeUppercase{\@title} \hfill}
  % Do nothing
\else
  \def\@oddhead{\small \MakeUppercase{\@shorttitle} \hfill}
\fi
\ifx \@surnamelist \@empty
  % Do nothing
\else
  \def\@evenhead{\small \MakeUppercase{\@surnamelist} \hfill}
\fi
\def\@oddfoot{\reset@font\hfil\thepage\hfil}%
\def\@evenfoot{\reset@font\hfil\thepage\hfil}%
\g@addto@macro\maketitle{\global\@specialpagetrue\gdef\@specialstyle{plain}}

%% Less hyphenation
\hyphenpenalty=1000  % Default: 50
%\tolerance=9000      % Default: 9999

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% This is all for the hyperref package and nice colors

%% The following conflicts with \texorpdfstring in section headers
% %% First, patch a bug from revtex4 to allow use of \nameref
% \usepackage{xpatch}% http://ctan.org/pkg/xpatch
% \makeatletter
% \xpatchcmd{\@ssect@ltx}{\@xsect}%
%   {\edef\@currentlabelname{#8}\@xsect}{}{}% Patch \<section>*
% \xpatchcmd{\@sect@ltx}{\@xsect}%
%   {\edef\@currentlabelname{#8}\@xsect}{}{}% Patch \<section>
% \makeatother

\definecolor{dodgerblue}{rgb}{0.12, 0.56, 1.0}
\definecolor{azure}{rgb}{0.0, 0.5, 1.0}
\definecolor{alizarincrimson}{rgb}{0.82, 0.1, 0.26}
\definecolor{mediumpurple}{rgb}{0.58, 0.44, 0.86}
\definecolor{lasallegreen}{rgb}{0.03, 0.47, 0.19}
\definecolor{my_gray}{rgb}{0,0,0}
\definecolor{uniwienblue}{HTML}{006699}
\definecolor{walesred}{HTML}{ff0038}
\definecolor{myorange}{HTML}{FF6C0C}
\definecolor{ferngreen}{HTML}{009246}
\definecolor{scarletred}{HTML}{CD212A}

\usepackage[colorlinks, plainpages=false,
hyperfigures=true]{hyperref}
% \usepackage[pagebackref=true, colorlinks, plainpages=false,
% hyperfigures=true]{hyperref}
% \renewcommand*{\backref}[1]{}
% \renewcommand*{\backrefalt}[4]{%
%   \ifcase #1 \or (Cited on p.~#2.) \else %
%   (Cited on pp.~#2.) \fi %
% }
\hypersetup{linkcolor=dodgerblue}
\hypersetup{citecolor=CiteColor}
\hypersetup{urlcolor=dodgerblue}
\hypersetup{setpagesize=false}
% \hypersetup{unicode} % Clashes with '\G' command defined in Macros
\hypersetup{pdfborder=0 0 0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatother

%\numberwithin{equation}{section}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

